Keck ESI Observations of Metal-Poor Damped Lyman-{\alpha} Systems

We present the first results from a survey of SDSS quasars selected for strong H I damped Lyman-{\alpha} (DLA) absorption with corresponding low equivalent width absorption from strong low-ion transitions (e.g. C II {\lambda}1334 and Si II {\lambda}1260). These metal-poor DLA candidates were selected from the SDSS DR5 quasar spectroscopic database, and comprise a large new sample for probing low metallicity galaxies. Medium-resolution echellette spectra from the Keck ESI spectrograph for an initial sample of 35 systems were obtained to explore the metal-poor tail of the DLA distribution and to investigate the nucleosynthetic patterns at these metallicities. We have estimated saturation corrections for the moderately under-resolved spectra, and systems with very narrow Doppler parameter (b \le 5 km s-1) will likely have underestimated abundances. For those systems with Doppler parameters b > 5 km s-1, we have measured low metallicity DLA gas with [X/H] < -2.4 for at least one of C, O, Si, or Fe. Assuming non-saturated components, we estimate that several DLA systems have [X/H] < -2.8, including five DLA systems with both low equivalent widths and low metallicity in transitions of both C II and O I. All of the measured DLA metallicities, however, exceed or are consistent with a metallicity of at least 1/1000 of solar, regardless of the effects of saturation in our spectra. Our results indicate that the metal-poor tail of galaxies at z \sim 3 drops exponentially at [X/H]< -3. The observed ratio of [C/O] for values of [O/H] < -2.5 exceeds values seen in moderate metallicity DLA systems, and also exceeds theoretical nucleosynthesis predictions for higher mass Population III stars.

==> tab_metalpoor.tex <==
 
 
\begin{deluxetable}{ccc}
\tablewidth{0pc}
\tablecaption{SDSS-DR5 Metal-Poor DLA Candidates\label{tab:candidates}}
\tabletypesize{\footnotesize}
\tablehead{\colhead{QSO} &
\colhead{$z_{\rm abs}$} &
\colhead{log $N_{\rm HI}$} }
\startdata
J001115.23$+14$4601& 3.612&20.65\\
J001134.52$+15$5137& 4.317&20.50\\
J001328.21$+13$5828.0& 2.612&20.10\\
J003749.19$+15$5208& 3.479&20.35\\
J012211.11$+15$0914.3& 3.519&20.45\\
J012403.77$+00$4432& 3.077&20.30\\
J014609.33$-09$2918& 3.680&20.25\\
J032226.09$-05$5824& 3.763&20.30\\
J033119.66$-07$4143& 4.192&20.65\\
J034300.88$-06$2229.9& 3.511&20.15\\
J073146.99$+36$4346& 3.591&20.80\\
J073149.51$+28$5448& 2.686&20.55\\
J073823.94$+34$0303.8& 3.817&20.15\\
J073938.85$+30$5951& 3.355&20.10\\
J074145.00$+21$5932.9& 2.578&20.80\\
J074713.25$+17$5948.2& 3.574&20.45\\
J074758.56$+29$3315.9& 2.813&20.15\\
J074856.03$+22$2953.3& 2.982&20.40\\
J075017.49$+40$5825& 2.792&20.20\\
J075054.84$+35$4240& 2.997&19.50\\
J075113.05$+31$2037.9& 3.384&20.45\\
J075155.10$+45$1619.6& 2.681&20.55\\
J075155.10$+45$1619.6& 3.046&20.45\\
J075155.10$+45$1619.6& 2.929&20.35\\
J075612.87$+29$1844.7& 3.672&20.20\\
J081110.32$+28$3814.1& 2.433&20.65\\
J081114.33$+39$3633& 2.651&20.95\\
J081114.33$+39$3633& 3.042&21.05\\
J081251.95$+20$0723.5& 2.548&21.10\\
J081332.61$+44$4813.1& 3.208&20.80\\
J081333.32$+35$0810& 4.303&20.35\\
J081427.60$+51$4516.4& 3.179&20.40\\
J081502.70$+06$2221.4& 2.775&19.75\\
J081813.14$+07$2054.9& 4.041&20.50\\
J082101.80$+03$4303.8& 3.559&20.35\\
J082204.68$+39$3722.9& 2.510&20.15\\
J082340.48$+34$2753.0& 3.845&20.05\\
J082401.62$+31$3113.6& 2.835&20.55\\
J082544.62$+33$3208& 2.485&20.70\\
J082857.48$+20$5243.7& 2.226&20.60\\
J082939.30$+07$0844.7& 3.426&20.25\\
J082939.30$+07$0844.7& 3.317&20.40\\
J083047.07$+51$1025.6& 2.805&20.15\\
J083102.55$+33$5803.1& 2.302&20.40\\
J083103.01$+52$3533& 3.868&20.45\\
J083122.57$+40$4623.4& 4.340&20.70\\
J083234.68$+31$5418.9& 2.485&20.30\\
J083328.06$+08$1317.5& 2.504&20.05\\
J083338.35$+42$0143.9& 3.713&20.20\\
J083400.49$+39$4216.9& 2.858&20.70\\
J083429.44$+21$4024.7& 3.711&20.65\\
J083436.69$+23$0628.8& 2.778&20.50\\
J083920.52$+35$2459.3& 4.285&20.40\\
J084249.02$+23$5204.7& 2.697&19.90\\
J084346.45$+29$0811.7& 3.027&19.55\\
J084426.10$+42$1646.5& 2.324&20.50\\
J084438.63$+46$2425& 3.335&20.75\\
J084438.63$+46$2425& 2.952&20.30\\
J084627.84$+08$0051.7& 4.739&20.15\\
J084719.12$+09$4323.4& 2.177&20.25\\
J085031.57$+35$5428.5& 3.893&20.20\\
J085323.22$+41$5121.3& 2.906&20.20\\
J085430.18$+00$4213.6& 3.691&20.35\\
J085534.79$+28$0018.4& 3.480&21.05\\
J085807.78$+40$4722.3& 2.974&20.55\\
J085853.98$+31$2639.4& 2.826&20.25\\
J090029.53$+43$0053& 4.264&20.50\\
J090333.55$+26$2836.3& 3.077&20.15\\
J090442.50$+41$5906.0& 3.567&19.75\\
J090832.28$+06$5853.8& 2.571&19.85\\
J091002.76$+42$2023.5& 2.374&19.85\\
J091016.79$+57$5331& 3.948&20.45\\
J091034.94$+52$1811& 3.423&20.10\\
J091046.67$+10$2629.9& 2.398&20.45\\
J091249.15$+07$5205.0& 3.434&19.85\\
J091859.43$+06$0833.6& 2.647&20.10\\
J092222.86$+31$4612.2& 3.067&20.35\\
J092222.86$+31$4612.2& 3.864&20.05\\
J092459.91$+09$5103.4& 3.340&20.90\\
J092814.93$+09$3955.2& 2.910&20.70\\
J093019.58$+42$3803.9& 3.610&20.20\\
J093032.42$+47$2021& 3.063&20.10\\
J093529.11$+07$3737.8& 2.869&19.80\\
J093746.47$+11$4038.4& 3.731&20.20\\
J093949.43$+33$5548.3& 3.726&19.85\\
J094050.44$+46$1730.5& 2.844&20.10\\
J094054.56$+05$4903.5& 2.578&20.70\\
J094100.99$+56$2843& 2.438&20.25\\
J094102.50$+56$0706.5& 2.811&20.20\\
J094108.36$+59$4725& 3.977&20.10\\
J094113.55$+11$4532.2& 2.289&20.15\\
J094149.45$+29$3343.3& 3.128&20.00\\
J094334.38$+05$1039.9& 2.926&20.00\\
J094337.29$+28$0135.9& 2.658&20.05\\
J094350.76$+42$5305.4& 3.176&20.55\\
J095037.09$+50$1925.5& 2.981&20.65\\
J095218.34$+09$2240.6& 2.800&20.20\\
J095436.32$+30$0336.1& 2.947&20.05\\
J095542.12$+41$1655.2& 3.277&20.30\\
J095604.43$+34$4415.5& 2.902&20.15\\
J100122.49$+48$5300.8& 3.026&20.40\\
J100151.45$+03$4301.5& 3.077&20.30\\
J100212.57$+44$0743.5& 2.355&20.40\\
J100321.11$+55$2059.4& 2.502&20.60\\
J100416.13$+43$4739.1& 4.474&21.00\\
J101049.63$+13$2746.8& 3.764&20.25\\
J101049.63$+13$2746.8& 3.334&19.90\\
J101107.98$+55$3407.0& 3.202&20.10\\
J101253.58$+10$5348.5& 2.894&20.35\\
J101336.33$+42$4026.5& 4.800&20.40\\
J101601.50$+40$4052.8& 2.816&20.05\\
J101821.67$+06$4434.4& 2.526&20.20\\
J102001.19$+39$2557.4& 2.661&20.55\\
J102301.01$+07$0918.2& 3.378&20.45\\
J102408.15$+49$0307.6& 3.924&20.50\\
J102619.09$+61$3628& 3.403&20.20\\
J102737.91$+48$0606.0& 3.700&20.50\\
J102846.92$+13$3936.2& 2.913&20.35\\
J102846.92$+13$3936.2& 3.290&20.15\\
J103126.13$+40$5532.5& 2.571&20.40\\
J103212.88$+12$0612.8& 2.772&20.25\\
J103401.75$+62$4214& 3.779&20.20\\
J103724.40$+01$3933& 2.704&20.45\\
J103751.06$+09$1035.0& 2.612&19.65\\
J103751.06$+09$1035.0& 2.899&20.00\\
J104002.51$+31$0449.9& 3.218&20.55\\
J104056.01$+45$3209.0& 3.574&20.05\\
J104302.43$+31$2434.0& 3.061&20.15\\
J104320.15$+50$1413& 3.195&20.10\\
J104328.08$+43$0620.6& 2.911&19.75\\
J104349.36$+61$5108& 2.786&20.80\\
J104448.78$+42$3509.3& 3.869&19.85\\
J104501.44$+50$4045.9& 3.949&20.35\\
J104600.41$+06$1054.1& 3.593&20.75\\
J104601.38$+53$2753.4& 2.630&19.95\\
J104810.81$+57$5526& 2.762&20.40\\
J104826.03$+39$1110.4& 2.297&20.55\\
J104914.73$+34$0210.9& 3.100&19.90\\
J105043.01$+30$0503.2& 2.796&20.80\\
J105123.03$+35$4534.3& 4.345&20.55\\
J105123.03$+35$4534.3& 3.903&20.50\\
J105320.40$+06$3747.9& 2.769&19.85\\
J105423.31$+13$0803.1& 3.129&20.20\\
J105430.07$+49$1947.1& 2.923&20.30\\
J105430.07$+49$1947.1& 3.391&20.50\\
J105623.88$+12$5414.3& 3.106&19.95\\
J105640.29$+07$5629.0& 3.461&20.35\\
J110001.49$+30$1215.1& 3.062&20.20\\
J110104.63$+14$1849.3& 3.113&19.70\\
J110622.99$+01$3055.5& 2.932&20.35\\
J110657.83$+08$1643.3& 3.368&19.50\\
J110855.47$+12$0953.3& 3.393&20.45\\
J110929.82$+58$2945& 2.454&20.20\\
J110931.69$+46$4048.0& 3.070&20.10\\
J111151.60$+13$3235.9& 2.270&20.50\\
J111224.18$+00$4630& 3.794&20.45\\
J111401.47$-00$5321& 4.265&20.05\\
J111427.68$+10$2840.8& 2.949&20.90\\
J111450.19$+45$2027.7& 2.804&20.10\\
J111511.65$+14$4512.1& 3.255&20.45\\
J112120.04$+35$4920.7& 2.940&20.00\\
J112121.63$+15$3201.4& 2.883&19.85\\
J112238.63$+45$4021.6& 3.245&20.10\\
J112300.25$+05$2451& 3.265&20.00\\
J113120.08$+38$3156.2& 3.541&19.80\\
J113534.55$+34$4433.8& 3.242&20.05\\
J113621.05$+00$5021& 2.362&19.90\\
J113657.24$+43$3402.9& 3.225&20.35\\
J113703.19$+10$4312.1& 3.764&19.90\\
J113805.24$+13$0332.6& 3.024&20.30\\
J114015.20$+15$0430.7& 2.848&20.10\\
J114514.05$+52$0154& 3.345&20.35\\
J114534.27$+49$3559.0& 2.287&19.80\\
J114623.61$+14$5523.6& 2.337&20.10\\
J114651.21$+47$1732.5& 2.675&20.15\\
J114709.26$+13$2118.3& 2.368&20.05\\
J115422.17$+53$5957.9& 2.422&20.25\\
J115422.17$+53$5957.9& 2.473&20.60\\
J115659.59$+55$1308.1& 2.491&20.55\\
J115809.39$+63$4252& 3.510&20.20\\
J120018.82$+10$5759.4& 3.343&20.05\\
J120450.61$+02$2118& 2.754&20.30\\
J120501.98$+58$5522& 2.694&21.05\\
J120525.27$+50$2355& 2.967&20.45\\
J120633.18$+44$5040.1& 2.584&20.50\\
J120816.46$+46$0440.0& 3.519&20.95\\
J120922.81$+12$5748.2& 3.233&20.10\\
J120949.74$+45$3400.4& 2.708&20.50\\
J121038.60$+56$0301.8& 3.474&20.15\\
J121504.99$+13$4135.4& 2.972&20.35\\
J121537.78$+54$5937.1& 3.933&19.85\\
J121613.65$+43$5024.3& 2.968&20.25\\
J121643.74$+62$4051& 3.317&20.25\\
J121646.20$+43$1921.6& 3.038&20.35\\
J121752.45$+08$5319.3& 3.390&21.45\\
J121915.70$+10$2449.4& 2.973&20.35\\
J121928.92$+16$0357.1& 3.005&20.30\\
J122008.93$+34$3642.3& 3.782&19.85\\
J122008.93$+34$3642.3& 3.503&20.25\\
J122021.39$+09$2135.7& 3.307&20.25\\
J122021.39$+09$2135.7& 3.305&20.40\\
J122042.00$+44$4218.2& 4.574&20.45\\
J122055.83$+66$0157& 3.779&20.20\\
J122330.30$+53$4850.1& 3.267&20.40\\
J122727.24$+57$0142.7& 3.272&20.25\\
J122844.82$+15$2402.4& 3.234&20.10\\
J123034.09$+51$0850.8& 2.769&20.50\\
J123116.08$+41$1337.3& 3.433&20.05\\
J123302.74$+09$4144.2& 3.406&20.60\\
J123556.86$+55$0826.7& 3.435&20.15\\
J123625.75$+36$0744.1& 3.507&20.30\\
J123706.53$+36$1516.9& 3.641&20.20\\
J123731.69$+57$4908.0& 2.732&20.35\\
J123937.17$+67$4020& 4.255&20.20\\
J124351.48$+45$3257.2& 2.623&20.45\\
J124659.55$+42$1735.4& 2.492&20.25\\
J124748.44$+04$2627& 2.422&20.25\\
J124830.64$+49$1400.2& 3.033&20.70\\
J125125.36$+41$2000.4& 2.730&21.00\\
J125319.14$+54$4954.6& 2.717&19.95\\
J125426.69$+41$2715.4& 2.754&20.20\\
J125743.51$+34$1520.9& 3.339&20.40\\
J125832.14$+29$0903.1& 3.066&20.10\\
J130049.59$+05$1339.2& 2.938&20.15\\
J130124.46$-01$5407.4& 2.526&20.75\\
J130215.72$+55$0553.4& 4.016&20.20\\
J130259.60$+43$3504.5& 3.346&20.40\\
J130501.32$+47$2824.1& 3.450&19.65\\
J130548.92$+29$0228.1& 2.385&20.30\\
J130719.29$+11$5218.8& 2.774&20.50\\
J130918.12$+40$2918.4& 2.889&20.10\\
J131246.45$+12$2930.2& 3.177&20.25\\
J131550.83$+57$2902.1& 2.873&20.60\\
J131808.76$+12$5334.8& 3.619&20.10\\
J131821.04$+41$3254.2& 2.947&20.55\\
J131917.78$+44$1201.4& 3.796&20.10\\
J132005.97$+13$1015.3& 2.673&20.30\\
J132009.70$+50$5058.5& 3.206&20.30\\
J132009.70$+50$5058.5& 3.513&20.15\\
J132012.88$+13$2409.4& 2.616&19.65\\
J132106.06$+62$3629.7& 4.131&20.30\\
J132512.49$+11$2329.7& 4.131&20.10\\
J132554.12$+12$5546.5& 3.550&20.40\\
J132605.10$+49$1448.4& 2.365&20.35\\
J132729.75$+48$4500.9& 2.445&20.80\\
J132729.75$+48$4500.9& 2.608&20.35\\
J132914.32$+41$0727.9& 3.692&20.05\\
J133030.25$+49$2718.6& 3.824&20.30\\
J133146.21$+48$3826.3& 3.240&20.95\\
J133146.21$+48$3826.3& 3.692&21.15\\
J133250.09$+46$5108.7& 4.647&20.75\\
J133326.31$+46$3143.3& 3.055&20.60\\
J133326.31$+46$3143.3& 3.168&20.40\\
J133448.70$+52$1317.9& 3.441&19.75\\
J133628.67$+60$2001& 2.808&20.55\\
J133701.39$-02$4630& 2.687&20.60\\
J133922.30$+46$2749.2& 2.830&20.05\\
J134107.26$-03$0342& 2.756&20.40\\
J134134.19$+01$4157& 3.631&20.60\\
J134216.12$+66$0727& 3.034&20.70\\
J134440.06$+28$3100.6& 3.360&20.20\\
J134637.94$+56$4915.6& 3.428&20.15\\
J134708.33$+52$5522& 2.729&20.55\\
J134759.60$+02$1308& 3.207&20.40\\
J134800.16$-02$2216& 3.040&20.85\\
J134820.86$+24$3707.9& 2.544&20.05\\
J134826.81$+36$1147.9& 3.218&20.70\\
J134939.78$+12$4230.7& 3.331&19.95\\
J134939.78$+12$4230.7& 3.492&20.40\\
J134939.78$+12$4230.7& 3.744&20.30\\
J135005.38$+66$1423& 2.365&20.60\\
J135018.86$-03$1047& 2.820&21.15\\
J135018.86$-03$1047& 2.744&20.30\\
J135044.21$+59$5205& 2.756&20.75\\
J135718.05$+50$2458.3& 2.640&20.05\\
J135842.92$+65$2236& 3.069&20.30\\
J140243.97$+59$0958& 3.779&21.70\\
J140404.64$+03$1403& 4.462&20.30\\
J140529.01$+06$3514.0& 3.649&19.95\\
J140709.34$+01$2420& 2.711&20.50\\
J140739.38$+60$3036.2& 4.663&20.30\\
J140802.98$+53$5154.2& 3.461&20.10\\
J140805.68$+13$0956.7& 2.669&20.10\\
J140817.27$+40$1155.3& 2.743&20.45\\
J140906.47$+38$5350.3& 2.825&20.70\\
J140931.62$+53$1146.7& 3.155&20.25\\
J141348.53$+44$5156.5& 3.315&19.85\\
J141919.45$+57$4514& 2.978&20.25\\
J142014.99$+40$4252.4& 3.562&20.05\\
J142025.75$+61$5510& 3.710&20.25\\
J142034.42$+06$4358.8& 3.285&20.05\\
J142239.88$+42$0220.3& 2.870&20.05\\
J142301.64$+07$5803.7& 2.908&20.15\\
J142325.92$+13$0300.6& 4.860&19.85\\
J142352.24$+40$4604.4& 2.789&20.15\\
J142403.82$+09$1351.8& 2.321&20.20\\
J142422.69$+13$1231.4& 3.353&19.85\\
J142610.52$+02$2052.9& 2.998&20.20\\
J142705.86$+33$0817.9& 4.093&20.25\\
J142921.87$+32$0624.6& 2.437&20.20\\
J143006.42$-01$2020& 3.115&20.50\\
J143007.35$+48$3052.9& 3.600&20.70\\
J143327.40$+48$2354.1& 3.213&20.15\\
J143408.31$+23$2229.9& 3.672&20.25\\
J143556.32$+43$5204.4& 4.050&20.45\\
J143638.02$+50$5107& 3.462&20.25\\
J144046.51$+51$2654.3& 3.498&20.15\\
J144051.89$+06$3709.6& 2.509&21.35\\
J144051.89$+06$3709.6& 2.823&20.30\\
J144059.63$+42$0404.1& 2.555&20.10\\
J144101.19$+55$5223.0& 2.905&20.30\\
J144101.19$+55$5223.0& 2.938&20.90\\
J144234.85$+44$2833.5& 2.915&20.90\\
J144420.79$+38$0000.5& 3.942&20.60\\
J144456.23$+32$4725.7& 3.645&20.40\\
J144559.71$+37$2317.1& 3.598&19.85\\
J144617.35$-01$0131& 3.710&20.30\\
J145214.96$+38$2632.6& 2.657&20.40\\
J145247.72$+11$5620.1& 3.679&20.15\\
J145543.12$+49$1703.3& 3.373&20.35\\
J145624.66$+04$0741.0& 2.673&20.35\\
J145646.79$+46$4933.8& 3.401&20.70\\
J150027.89$+43$4200.8& 4.096&20.00\\
J150056.04$+38$2332.1& 2.586&20.05\\
J150056.04$+38$2332.1& 2.315&19.75\\
J150643.81$+53$3134.3& 3.227&19.70\\
J150802.29$+43$0645.4& 4.349&20.10\\
J150823.16$+45$2922.0& 2.651&19.55\\
J151037.17$+34$0220.6& 2.323&21.00\\
J151428.11$+49$4235.9& 2.627&20.00\\
J151602.33$+44$3233& 3.615&20.35\\
J151625.68$+32$5207.9& 2.326&19.95\\
J151931.27$+41$4531.9& 2.167&20.30\\
J152046.46$+52$5923& 2.765&20.55\\
J152247.77$+40$2411.0& 2.559&20.55\\
J152413.35$+43$0537.4& 2.871&20.40\\
J153024.15$+48$1416.3& 2.323&20.40\\
J153129.90$+45$1707.6& 4.085&20.30\\
J153648.72$+43$2154.2& 2.152&20.80\\
J153958.05$+50$3840.1& 3.286&20.35\\
J154114.92$+50$4353.6& 2.655&20.10\\
J154559.64$+40$1506.6& 3.733&20.75\\
J154841.76$+35$2141.9& 4.549&20.10\\
J154905.84$+35$2020.5& 2.711&20.00\\
J154906.71$+46$0756.7& 3.646&20.20\\
J155120.79$+32$0155.1& 3.012&19.65\\
J155142.02$+33$5351.1& 2.471&20.05\\
J155248.02$+56$0328& 3.555&20.25\\
J155639.53$+31$2739.9& 3.486&20.35\\
J155738.39$+23$2057.5& 3.538&20.50\\
J155800.10$+31$1438.2& 3.171&19.70\\
J160244.76$+32$4036.6& 2.975&20.35\\
J160329.14$+09$0218.2& 4.518&20.05\\
J160641.00$+29$1919.3& 4.002&20.15\\
J161018.06$+25$3600.9& 3.453&20.90\\
J161105.64$+08$4435.4& 3.777&20.25\\
J161119.57$+44$1144& 3.981&20.70\\
J161559.52$+23$3203.9& 3.978&19.90\\
J162336.73$+31$5225.8& 2.503&20.50\\
J162445.66$+32$0722.3& 3.716&20.05\\
J162722.85$+44$4134& 2.201&20.05\\
J163259.68$+39$0423.0& 2.707&20.25\\
J163411.82$+21$5325.0& 4.083&20.65\\
J163603.35$+38$1122.3& 3.542&20.45\\
J163609.72$+31$3827.9& 3.419&20.30\\
J163712.01$+38$1135.2& 3.140&19.60\\
J163714.69$+39$5706.8& 3.241&20.20\\
J163747.58$+29$0135.2& 3.504&20.35\\
J163809.01$+32$3955.2& 2.351&20.45\\
J163809.01$+32$3955.2& 2.351&20.45\\
J163816.30$+24$5515.1& 2.796&20.05\\
J164810.07$+26$0211.3& 2.953&20.45\\
J165001.22$+34$3003.6& 3.812&20.00\\
J165354.61$+40$5402.1& 4.574&20.35\\
J165408.17$+35$0954& 2.407&20.95\\
J165436.85$+22$2733.7& 4.007&20.35\\
J165716.50$+32$4849& 2.197&19.80\\
J165722.24$+33$3540& 2.392&20.15\\
J165902.11$+27$0935.1& 4.494&20.05\\
J170423.44$+32$1313.9& 2.667&20.10\\
J170839.74$+30$0116.0& 3.475&20.65\\
J170931.01$+34$1731& 3.013&20.45\\
J171014.51$+59$2326& 4.017&20.15\\
J171509.96$+29$4555.0& 4.237&20.10\\
J171719.45$+58$0218& 3.046&20.40\\
J211450.33$-06$3257& 4.127&20.85\\
J222509.19$-00$1406& 4.219&20.55\\
J222644.78$+00$5019.8& 2.488&20.15\\
J223447.03$-09$3759& 2.978&20.20\\
J223619.19$+13$2620.3& 2.552&20.10\\
J224147.76$+13$5202.7& 3.655&20.20\\
J224147.76$+13$5202.7& 3.458&19.90\\
J224246.53$+14$0346.3& 2.524&20.20\\
J224255.52$+12$4225.6& 3.890&20.20\\
J224255.52$+12$4225.6& 3.717&20.30\\
J224630.86$+13$1706& 3.606&21.10\\
J224823.60$+12$5711& 3.016&20.30\\
J225246.44$+14$2525.7& 4.749&20.20\\
J231858.57$-00$5049.6& 3.002&20.05\\
J232025.08$-10$4226& 3.611&20.65\\
J232025.08$-10$4226& 3.431&20.30\\
J233756.58$-10$2000.1& 2.346&20.00\\
J233838.22$-00$3513.7& 2.372&19.90\\
J233838.22$-00$3513.7& 2.372&19.90\\
J235028.85$+15$1626.7& 2.669&20.40\\
\enddata
\tablecomments{{} List of all candidate metal-poor DLAs flagged by Prochaska and collaborators from their analysis of the SDSS-DR5.  We caution that many of these will not be bona-fide DLAs.}
\end{deluxetable}
 
\clearpage

